Conservative Discontinuous Galerkin Schemes for Nonlinear Fokker-Planck Collision Operators

We present a novel discontinuous Galerkin algorithm for the solution of a class of Fokker-Planck collision operators. These operators arise in many fields of physics, and our particular application is for kinetic plasma simulations. In particular, we focus on an operator often known as the `Lenard-Bernstein,' or `Dougherty,' operator. Several novel algorithmic innovations are reported. The concept of weak-equality is introduced and used to define weak-operators to compute primitive moments needed in the updates. Weak-equality is also used to determine a reconstruction procedure that allows an efficient and accurate discretization of the diffusion term. We show that when two integration by parts are used to construct the discrete weak-form, and finite velocity-space extents are accounted for, a scheme that conserves density, momentum and energy exactly is obtained. One novel feature is that the requirements of momentum and energy conservation lead to unique formulas to compute primitive moments. Careful definition of discretized moments also ensure that energy is conserved in the piecewise linear case, even though the $v^2$ term is not included in the basis-set used in the discretization. A series of benchmark problems are presented and show that the scheme conserves momentum and energy to machine precision. Empirical evidence also indicates that entropy is a non-decreasing function. The collision terms are combined with the Vlasov equation to study collisional Landau damping and plasma heating via magnetic pumping. We conclude with an outline of future work, in particular with some indications of how the algorithms presented here can be extended to use the Rosenbluth potentials to compute the drag and diffusion coefficients.

==> novelty.tex <==
This paper presents a novel discontinuous Galerkin scheme to evolve a nonlinear Fokker-Planck operator for use in kinetic simulations of plasmas. Often collisions are crucial to explain the observed physics in many plasma problems. The scheme presented here conserve density, momentum and energy. Numerically, we also observe that the entropy increases monotonically. The scheme is implemented in the \gke\ code and is available as a open-source package.

The scheme presented here is unique. It uses a recovery method to compute the second derivatives needed in discretizing the diffusion terms. Two integrations by parts are needed to get momentum and energy conservation. A new concept of weak equality is introduced that allows a consistent defition of moments needed in the updates. Several examples are shown, including the collisionless terms, spanning physics from neutral to fully kinetic, electromagnetic plasmas.

Many of the ideas presented here can have an impact on fields outside plasma-physics. For example, the obervation that moments need to be computed in a particular manner can be used to compute alias-free methods for fluid equations. The idea of weak-equality is very general and can be used in constructing other novel solvers for PDEs and ODEs.

\newpage

Several novel algorithmic innovations are reported here. In particular:
\begin{itemize}\cramplist
    \item The definition of weak-equality and its application to weak-division and construction of the discrete diffusion term is crucial. See Section~\thinspace\ref{sec:weakeq}. This allows an alias-free and consistent approach to computing the primitive moments needed in the Fokker-Planck operator. The definition of weak-equality is also used to describe the reconstruction process needed in the diffusion term.
    \item The use of two integration by parts is required to ensure that momentum and energy, in addition to density, are conserved by the discrete scheme. Without the second integration by parts jumps in the distribution function would be picked up and make the scheme non-conservative. Further, the diffusion term in the FPO requires accounting for finite velocity space extents. See Scheme C, \eqr{\ref{eq:schemec}}, and the conservation proofs in Section~\ref{sec:scheme-theory}. Interestingly, the requirements on momentum and energy conservation, combined with finite-velocity extents, also lead to a unique and consistent method to determine the drift-velocity and thermal speeds. 
    \item For piecewise linear basis sets energy conservation can be obtained by carefully defining the ``star'' moments; see Proposition~\ref{prop:sc_erCons_p1}. Naively, one may have assumed that $\vv^2$ must be included in the basis set. However, with the definition of the star-moments we can continue to conserve energy exactly even when using $p=1$ basis.
\end{itemize}

\newpage

No conflicts of interests are reported.
